In-Place Zero-Space Memory Protection for CNN

Convolutional Neural Networks (CNN) are being actively explored for safety-critical applications such as autonomous vehicles and aerospace, where it is essential to ensure the reliability of inference results in the presence of possible memory faults. Traditional methods such as error correction codes (ECC) and Triple Modular Redundancy (TMR) are CNN-oblivious and incur substantial memory overhead and energy cost. This paper introduces in-place zero-space ECC assisted with a new training scheme weight distribution-oriented training. The new method provides the first known zero space cost memory protection for CNNs without compromising the reliability offered by traditional ECC.

==> Makefile <==
SOURCES	= \
	paper.tex

.PHONY: default all clean

default:
	pdflatex paper.tex

all:  
	pdflatex paper.tex
	-	bibtex paper
	pdflatex paper.tex
	pdflatex paper.tex
	thumbpdf paper.pdf
	pdflatex paper.tex

clean:
	-rm -rf paper.synctex.gz paper.out paper.tpt paper.aux paper.bbl paper.blg paper.dvi *.log paper.ps *.txt *~

sources:
	@echo  ${SOURCES}

